Reasoning about Intuitionistic Computation Tree Logic

In this paper, we define an intuitionistic version of Computation Tree Logic. After explaining the semantic features of intuitionistic logic, we examine how these characteristics can be interesting for formal verification purposes. Subsequently, we define the syntax and semantics of our intuitionistic version of CTL and study some simple properties of the so obtained logic. We conclude by demonstrating that some fixed-point axioms of CTL are not valid in the intuitionistic version of CTL we have defined.

==> eptcsdata.tex <==
\providecommand{\firstpage}{42}
\providecommand{\publicationstatus}{A. Ferrando, R.C. Cardoso (Eds.): Third Workshop on\\ Agents and Robots for reliable Engineered Autonomy 2023 (AREA'23)\\
EPTCS 391, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.391.6}{10.4204/EPTCS.391.6}}

